AutoGNN: End-to-End Hardware-Driven Graph Preprocessing for Enhanced GNN Performance

Graph neural network (GNN) inference faces significant bottlenecks in preprocessing, which often dominate overall inference latency. We introduce AutoGNN, an FPGA-based accelerator designed to address these challenges by leveraging FPGA's reconfigurability and specialized components. AutoGNN adapts to diverse graph inputs, efficiently performing computationally intensive tasks such as graph conversion and sampling. By utilizing components like adder trees, AutoGNN executes reduction operations in constant time, overcoming the limitations of serialization and synchronization on GPUs. AutoGNN integrates unified processing elements (UPEs) and single-cycle reducers (SCRs) to streamline GNN preprocessing. UPEs enable scalable parallel processing for edge sorting and unique vertex selection, while SCRs efficiently handle sequential tasks such as pointer array construction and subgraph reindexing. A user-level software framework dynamically profiles graph inputs, determines optimal configurations, and reprograms AutoGNN to handle varying workloads. Implemented on a 7$n$m enterprise FPGA, AutoGNN achieves up to 9.0$\times$ and 2.1$\times$ speedup compared to conventional and GPU-accelerated preprocessing systems, respectively, enabling high-performance GNN preprocessing across diverse datasets.

==> discussion.tex <==
\markerCommentOnly[-2]{\shortstack{C\#Q2, D\#Q1, E\#D1, E\#Q1: Is \\ preprocessing from scratch necessary?}}
\markerCommentOnly[60]{\shortstack{B\#Q2, E\#D4, E\#Q3: \\ Sensitivity analysis}}
\hlF{\noindent\textbf{Incremental preprocessing.}
Maintaining an up-to-date graph is required in many real-time GNN applications since minor vertex updates can alter the overall topology and impact the accuracy of GNN models~\mbox{\cite{yin2023deltagnn}}.
% In addition, many GNN applications demand real-time integration of newly collected data~\mbox{\cite{sarkar2023flowgnn, shi2020point, shlomi2020graph}}.
The most widely used graph format, CSC, enables efficient traversal due to its compressed structure but requires global modifications for graph updates, making incremental updates infeasible.
% For example, inserting a single edge into a CSC-formatted graph involves: i) determining the insertion location, ii) shifting the index array, iii) inserting the new edge, and iv) updating subsequent pointers.
Several approaches have been proposed to mitigate the inefficiencies in CSC updates. These methods fall broadly into two categories. The first involves padding spaces within the CSC structure in advance, allowing storage of new edges without immediate restructuring~\mbox{\cite{de2019packed, wheatman2018packed, sha2017technical, islam2022vcsr}}. The second maintains an auxiliary edge list for newly added edges, linked to the original CSC-formatted graph using separate pointers~\mbox{\cite{macko2015llama, kumar2020graphone}}.
These approaches accelerate incremental updates by eliminating the need to reorganize the entire graph upon minor insertions. However, because they do not utilize fully compressed representations like CSC, they require additional pointer-chasing operations during graph traversal, reducing GNN model computation efficiency. Moreover, they periodically demand extensive operations, such as allocating new padding or merging the updates to the original graph, resulting in substantial tail latency.
According to our evaluations, these structures degrade GNN computation performance by 2$\times$ on average. Only the largest evaluated graph (TB) shows a 4\% performance gain; all other graphs suffer performance degradation.
}


\begin{figure}
  \vspace{0pt}
  \begin{subfigure}[t]{0.49\linewidth}
    \vspace{0pt}
    \centering
    \includegraphics[width=\linewidth]{figures/result_timeline-g}
    \vspace{-10pt}
    \caption{Time-series analysis.}\label{fig:result_timeline-g}
  \end{subfigure}%
  \begin{subfigure}[t]{0.49\linewidth}
    \vspace{0pt}
      \centering
      \includegraphics[width=\linewidth]{figures/result_mixed_1}
      \vspace{-10pt}
      \caption{Various graph pairs.}\label{fig:result_mixed_timeline}
  \end{subfigure}
  \vspace{-11pt}
  \caption{Consecutive inference using diverse graph.}\label{fig:result_timeline}
  \vspace{-10pt}
\end{figure}



% \hlF{\noindent\textbf{Incremental preprocessing.}
% GNNs frequently handle graphs with complex interconnections, where minor vertex updates can affect the overall topology. Ignoring such updates during inference negatively impacts accuracy~\mbox{\cite{yin2023deltagnn}}; thus, maintaining an up-to-date graph is critical. In addition, many GNN applications demand real-time integration of newly collected data~\mbox{\cite{sarkar2023flowgnn, shi2020point, shlomi2020graph}}, which places significant pressure on preprocessing performance.

% Although GNN inference typically employs the CSC format for efficient aggregation, its compressed structure inherently complicates incremental updates. For example, inserting a single edge into a CSC-formatted graph involves multiple sequential steps: i) determining the correct insertion location based on the destination vertex identifier (VID), ii) shifting the corresponding portion of the index array, iii) inserting the new edge into the appropriate position among existing edges sharing the same destination VID, and iv) updating subsequent pointers accordingly. Each insertion triggers these sequential operations, causing considerable overhead.

% Several approaches have been proposed to mitigate the inefficiencies in CSC updates. These methods fall broadly into two categories. The first involves allocating padding spaces within the CSC structure in advance, allowing storage of newly added edges without immediate restructuring~\mbox{\cite{de2019packed, wheatman2018packed, sha2017technical, islam2022vcsr}}. The second maintains an auxiliary edge list for newly added edges, linking it to the original CSC-formatted graph using separate pointers~\mbox{\cite{macko2015llama, kumar2020graphone}}.

% These approaches accelerate incremental updates by eliminating the need to reorganize the entire graph upon the insertion of a small number of edges, thus reducing the latency of graph conversion during GNN preprocessing. However, because these techniques do not utilize fully compressed representations like CSC, they require additional pointer chasing operations during graph traversal, reducing GNN model computation efficiency. Moreover, they periodically demand extensive operations, such as allocating new padding spaces or merging the auxiliary edge list into the original graph, resulting in substantial tail latency.

% According to our evaluations, these incremental update structures degrade GNN computation performance by an average factor of XX. Only the largest evaluated graph (TB) shows a XX-fold performance gain; all other graphs suffer performance degradation.
% }






% \begin{itemize}[leftmargin=*]
%   \item \khlc{정점-간 복잡한 연결관계를 갖고 있는 그래프의 특성 상, 일부 정점만이 변경되더라도 대부분의 정점들이 연산 결과에 영향을 받으며, 때문에 이를 고려하지 않으면 추론 시 정확도가 크게 감소함}\cite{yin2023deltagnn}\khlc{. 때문에 추론 시 최신의 그래프를 활용하는 것은 정확도를 유지를 위해 필수적임}.
%   \item \khlc{이외에도 실시간으로 새로운 그래프를 수집하고, 이에 대한 빠른 추론을 수행해야 하는 GNN 응용이 증가하고 있음에 따라}\cite{sarkar2023flowgnn}, \khlc{GNN의 전처리 연산시간은 추론 시 고려되어야 하는 주요 문제임.}
% \end{itemize}
% \begin{itemize}[leftmargin=*]
%   \item \khlc{GNN 모델 연산은 취합 (aggregation) 연산의 용이성을 위해 CSC 자료구조를 요구하나, CSC 자료구조는 그 압축된 형태로 인해 직접적인 변경이 어려움.}
%   \begin{itemize}[leftmargin=*]
%     \item \khlc{예를 들어, 기존의 CSC의 중간에 새로운 간선을 추가하기 위해선 삽입할 위치 탐색 (search), 공간 생성 (allocate), 추가 (insert), 자료구조 업데이트 (update)의 과정이 요구됨.}
%     \item \khlc{먼저, 추가하고 싶은 간선의 dst VID를 기준으로 CSC의 ptr 배열을 참조해 새로운 간선의 정보가 추가되어야 할 위치를 검색함.}
%     \item \khlc{이후, 간선 정보를 추가할 공간을 만들기 위해, 해당 dst VID의 범위 이후의 모든 간선의 index array를 복사하여 한 칸 오른쪽으로 이동시킴.}
%     \item \khlc{간선을 추가하기 위해선 추가하고자하는 간선과 같은 dst VID를 가진 기존의 간선들의 src VID들을 읽은 뒤, 정렬이 유지되는 위치를 찾아 새로운 간선 정보를 저장해야 함.}
%     \item \khlc{마지막으로, index array에 여유공간을 만들기 위해 오른쪽으로 한 칸 이동한 것을 고려하기 위해 삽입한 간선 이후의 대한 모든 ptr array 원소들에 1을 더해줌.}
%     \item \khlc{위의 과정은 추가해야 하는 모든 간선에 대해 수행되어야 하며, index array의 복사와 ptr array의 수정을 요구하기 때문에 순차적으로 수행되어야 함. 때문에 CSC 자료구조를 직접 수정하는 것은 매우 큰 오버헤드를 발생시킴.}
%   \end{itemize}
%   \item \khlc{Note: GNN의 학습 과정은 추론 과정과 달리 같은 그래프에 대해 다수번의 추론을 진행하는 특징을 갖고 있어, 전처리된 결과를 재활용할 수 있음.}
% \end{itemize

% \noindent\textbf{Training support.}
% Although AutoGNN is designed for inference, it can support GNN training. Training requires graph sampling, each followed by backpropagation steps which uses the CSR format. CSR generation can occur without modifying hardware logic by reversing VID concatenation order during the \texttt{Ordering} stage. However, training involves repeated inferences on the same graph, allowing partial reuse of preprocessing results (as a CSC). In contrast, inference needs to process new or updated graphs with minimal delay -- the focus of the work.

% Although AutoGNN is designed for inference, it can support GNN training. Training requires graph sampling, each followed by backpropagation steps depending on a CSR representation of sampled graph. Generating a CSR can occur without modifying hardware logic by reversing the order in which VIDs are concatenated during the \texttt{Ordering} stage (i.e., placing the source VID before destination VID). However, training involves repeated inferences on the same graph, allowing partial reuse of preprocessing results (as a CSC). In contrast, inference often needs to process new or updated graphs with minimal delay -- the focus of the work.

% Although AutoGNN is designed primarily for inference, it can also support GNN training. Training requires multiple rounds of graph sampling, each followed by additional backpropagation steps that depend on a CSR representation of the sampled graph. Generating a CSR can be done without modifying the hardware logic by reversing the order in which VIDs are concatenated during the \texttt{Ordering} stage (i.e., placing the source VID before the destination VID). However, training generally involves repeated inferences on the same graph, allowing partial reuse of preprocessing results (such as a CSC). In contrast, inference scenarios often need to process new or frequently updated graphs with minimal delay, which is the key focus of this work.

% AutoGNN's flexible hardware configuration further helps reduce preprocessing overhead by reallocating resources to handle the increased sampling load.


% \begin{itemize}[leftmargin=*]
%   \item \khlc{AutoGNN은 GNN의 추론 뿐만 아니라 학습 또한 지원이 가능함.}
%   \item \khlc{GNN 학습은 입력 그래프에 대해 다양한 batch를 활용한 추론을 진행하기 때문에 graph sampling을 반복적으로 수행해야 하며, 추가적인 back-propagation 연산을 위해 sampled 그래프의 CSR 형태를 추가로 요구한다는 특징을 가짐.}
%   \begin{itemize}[leftmargin=*]
%     \item \khlc{CSR의 생성은 \texttt{Ordering} 과정 중 VID의 concatenation을 반대로 (src VID를 먼저, dst VID를 나중) 함으로써 하드웨어 로직의 변경없이 가능함.}
%     \item \khlc{또한, AutoGNN은 늘어난 graph sampling의 비중에 맞는 최적의 하드웨어 구성을 제공함으로써 GNN 학습 과정의 전처리 시간을 최소화할 수 있음.}
%   \end{itemize}
%   \item \khlc{하지만, GNN의 학습은 추론과 달리 같은 입력 그래프에 대해 여러번 추론을 진행하기 떄문에 그래프의 전처리 결과 일부(e.g., 그래프의 CSC)를 캐싱하여 사용할 수 있음.}
%   \begin{itemize}[leftmargin=*]
%     \item \khlc{이에 따라 본 논문은 학습보단 추론의 시나리오에 집중함.}
%   \end{itemize}
% \end{itemize}

% The FPGA-based system has 12 GB of DRAM, supporting graphs up to 1.5B edges. Accelerator memory capacity grows (e.g., the H100 GPU can handle up to 20B edges \mbox{\cite{sahebi2023distributed,zhu2019aligraph}}), the design remains viable for large-scale applications. However, since each vertex or edge embedding can exceed several KB, so total embedding data may exceed on-board memory capacity. To address this, we store only the graph data on FPGA memory and stored large embeddings on host's main memory. Note that FPGA does not need embedding data while preprocessing GNN.
\markerCommentOnly[1]{\shortstack{A\#Q5: Large \\ graph support}}
\hlA{
  \noindent\textbf{Large graph support.}
The FPGA-based evaluation system, which includes 12GB of DRAM, supports graphs with up to 1.5B edges by storing only graph data on-device and offloading embeddings to host memory. This covers 90\% of real-world graphs \mbox{\cite{snapnets}}. As accelerator memory scales (e.g., the H100 GPU supports up to 20B edges~\mbox{\cite{sahebi2023distributed,zhu2019aligraph}}), AutoGNN remains a scalable solution.
}

% \hlA{
%   \noindent\textbf{Large graph support.}
%   The FPGA-based system used for evaluation contains 12 GB of DRAM, supporting graph datasets up to 1.5B edges.
%   This is possible because AutoGNN only stores the graph data and stores the large embeddings in host memory, which is usually several KB per edge or vertex.
%   Thus, AutoGNN can cover 98\% of major real-world graph datasets including large commercial graphs \mbox{\cite{snapnets}}.
%   Considering the increasing memory capacity of accelerators (e.g., the H100 GPU supports graphs up to 20B edges~\mbox{\cite{sahebi2023distributed,zhu2019aligraph}}), the proposed architecture remains suitable for large-scale applications.
% }

\markerCommentOnly[15]{\shortstack{B\#D1, B\#Q1: General \\ GNN model support}}
\hlB{
\noindent\textbf{General GNN model support.}
Since GNN preprocessing is decoupled from specific model architecture, AutoGNN supports a wide range of GNN models (e.g., GCN \mbox{\cite{kipf2016semi}}, GAT \mbox{\cite{velivckovic2017graph}}, GIN \mbox{\cite{xiyuan2022how}}) that rely on CSC/CSR formats, regardless of model depth.
Furthermore, with minimal modifications, AutoGNN can accommodate not only GraphSAGE but also various sampling strategies. Sampling methods are typically categorized into node-wise \mbox{\cite{hamilton2017inductive,jianfei2018stochastic}} and layer-wise sampling \mbox{\cite{ying2018graph,chen2018fastgcn,wenbing2018adaptive,difan2019layerdependent}}, depending on whether uni-random selection occurs after each node's or the entire layer's neighborhood exploration. The UPE of AutoGNN can accelerate both node- and layer-wise sampling by reordering graph traversal and uni-random selection within the controller.
Moreover, weight-based sampling \mbox{\cite{ying2018graph,wenbing2018adaptive,chen2018fastgcn}} can also benefit from AutoGNN by simply modifying the random number generation process; configuring the random number generation logic to assign subranges of the LSFR's output range in proportion to each element's weight.
}


% \hlB{
% \noindent\textbf{General GNN model support.}
% AutoGNN supports a wide range of GNN models, such as GCN\mbox{\cite{kipf2016semi}}, GAT\mbox{\cite{velivckovic2017graph}}, GIN\mbox{\cite{xiyuan2022how}} and others that rely on the CSC (or CSR) data structure, since GNN preprocessing is decoupled from the specific model architecture. This compatibility extends regardless of the depth of the GNN model. Furthermore, with minimal modifications, AutoGNN can accommodate not only GraphSAGE but also various sampling strategies.
% Sampling methods can largely be categorized into node-wise sampling \mbox{\cite{hamilton2017inductive,jianfei2018stochastic}} and layer-wise sampling \mbox{\cite{ying2018graph,chen2018fastgcn,wenbing2018adaptive,difan2019layerdependent}}, depending on whether the uni-random selection of the explored vertices is done after each neighborhood exploration or after the entire layer-wise exploration is completed.
% The UPE of AutoGNN accelerates the uni-random selection process, which is fundamental to both node-wise and layer-wise sampling techniques. To this end, AutoGNN can accelerate both sampling paradigms by reordering graph traversal and uni-random selection within the controller.
% It should be noted that, sampling techniques based on weights \mbox{\cite{ying2018graph,wenbing2018adaptive,chen2018fastgcn}} can also benefit from AutoGNN's acceleration simply by modifying the random number generation process; configuring the random number generation logic to assign subranges of the LSFR's output range in proportion to each element's weight.
% }

% \begin{itemize}[leftmargin=*]
%   \item \khlc{평가에 활용한 FPGA는 12GB의 DRAM을 활용하여 1.5B 크기의 그래프까지는 처리할 수 있음.}
%   \begin{itemize}[leftmargin=*]
%     \item \khlc{FPGA와 GPU 등 가속기들이 지원하는 DRAM의 크기는 계속하여 커지고 있는 추세이기 때문에, 최신 가속기 (e.g., H100 GPU)들은 20B 크기의 그래프까지 처리가 가능함.}
%     \item \khlc{대형 그래프 응용들}\cite{sahebi2023distributed,zhu2019aligraph} \khlc{또한 수 billion-scale 크기의 그래프를 고려하고 있기 때문에, 제안하는 가속기 디자인은 충분히 큰 그래프를 지원할 수 있음.}
%   \end{itemize}
%   \item \khlc{단, 그래프의 임베딩은 각 정점 혹은 간선마다 수 kB의 크기를 갖기 때문에, 그래프 자체 대비 훨씬 크며, 이는 AutoGNN은 물론, 다른 가속기들 또한 DRAM에 적재하기 어려움.}
%   \begin{itemize}[leftmargin=*]
%     \item \khlc{이를 해결하기 위해서 PCIe와 같은 고속 인터커넥트를 통한 호스트 메모리와의 통신이 필수적임.}
%   \end{itemize}
% \end{itemize}


\markerCommentOnly[8]{\shortstack{A\#Q2, D\#Q2: FPGA \\ reconfiguration overhead}}
\hlF{\noindent\textbf{Hardware reconfigure frequency.}
AutoGNN employs a cost function (cf. Section~\mbox{\ref{sec:dyn-reconfig}}) to trigger FPGA reconfiguration only when it reduces net execution time. In practice~\mbox{\cite{shi2020point,zhu2019aligraph,zhao2019intentgc}}, graph parameters like vertex and edge counts change gradually, making frequent reconfiguration unnecessary. First, when a single dynamic graph evolves gradually~\mbox{\cite{taobaodataset,feng2024comprehensive,zhu2019aligraph}}, hardware reconfiguration is beneficial only after substantial graph changes accumulate. In our evaluation datasets (SO and TB), only 12 and 6 reconfigurations were needed over 2000 and 100 days, respectively.
Second, when processing successive graphs with similar characteristics~\mbox{\cite{shi2020point,sarkar2023flowgnn,shlomi2020graph}}, a single hardware configuration remains effective across multiple runs. Consequently, AutoGNN reconfiguration occurs infrequently in real-world workloads, making its overhead negligible.}


% \hlF{\noindent\textbf{Hardware reconfigure frequency.}
% AutoGNN employs a cost function (cf. Section~\mbox{\ref{sec:dyn-reconfig}}) to evaluate the trade-off between potential performance gains and FPGA reconfiguration overhead, thus reconfiguring only when the net execution time is reduced. In practical scenarios~\mbox{\cite{shi2020point,zhu2019aligraph,zhao2019intentgc}}, key graph parameters such as vertex and edge counts typically undergo minimal changes, reducing the necessity for frequent reconfiguration. Two representative cases illustrate this principle. First, in scenarios involving a single, gradually evolving dynamic graph~\mbox{\cite{taobaodataset,feng2024comprehensive,zhu2019aligraph}}, hardware reconfiguration is beneficial only after substantial graph changes accumulate. For example, in our evaluation datasets (SO and TB), AutoGNN required reconfiguration 12 and 6 times during graph evolution periods of 2000 and 100 days, respectively.
% Second, in applications processing successive graphs with similar characteristics~\mbox{\cite{shi2020point,sarkar2023flowgnn,shlomi2020graph}}, the same hardware configuration remains effective across multiple runs. Consequently, AutoGNN reconfiguration occurs infrequently in real-world workloads, making its overhead negligible.}

% \noindent\textbf{Hardware reconfiguring overhead}
% AutoGNN uses a cost function (cf. Section {\ref{sec:dyn-reconfig}}) to balance performance gains against FPGA reprogramming overhead, reconfiguring only when execution time improves. In many scenarios {\cite{shi2020point, zhu2019aligraph, zhao2019intentgc}}, fluctuations in graph parameters (vertex/edge counts)  undergo only minor fluctuations, thereby minimizing the need for reconfiguration. For example, a gradually evolving dynamic graph {\cite{taobaodataset, feng2024comprehensive, zhu2019aligraph}} warrants reprogramming only after significant changes; with new but similar input graphs {\cite{shi2020point, sarkar2023flowgnn, shlomi2020graph}}, the same hardware configuration suffices across runs. In both cases, AutoGNN employs partial FPGA reconfiguration with pre-synthesized on-board bitstreams, cutting reprogramming time to about 0.2s, often negligible.

% \begin{itemize}[leftmargin=*]
%   \item \khlc{AutoGNN은 제안하는 cost 함수를 통해 재구성을 통해 얻을 수 있는 성능 이득을 정확히 모델링할 수 있으며, 따라서 재구성을 고려했을 때의 총 지연시간이 짧아지는 경우에만 재구성을 수행함.}
%   \item \khlc{추가로, 입력되는 그래프의 주요 특징은 크게 변하지 않음. 이는 응용의 성격에 따라 크게  두 가지 경우를 나누어 설명함.}
%   \item \khlc{첫째, 하나의 그래프가 계속 변화하는 경우 (dynamic graph)에는 그래프가 바뀔 때마다 재구성을 하지 않아도 괜찮음.}
%   \begin{itemize}[leftmargin=*]
%     \item \khlc{Taobao 그래프의 사례를 보면, 전처리 시간이 재구성으로 인해 10\% 이상의 이득을 보는 경우는 600시간 어치 업데이트가 축적된 이후부터임. 즉, 약 0.2초가 요구되는 재구성 과정의 오버헤드는 그 주기 대비 충분히 작음.}
%   \end{itemize}
%   \item \khlc{둘째, 자율 주행을 위한 point cloud 응용[??] 혹은 고에너지 물리학 응용[??]과 같이 매번 새로운 그래프가 들어오는 경우, 비록 그래프 자체는 매번 새로우나, 입력되는 그래프의 주요 특징들은 큰 편차를 가지지 않음.}
%   \begin{itemize}[leftmargin=*]
%     \item \khlc{최적의 하드웨어 구성을 결정하는 가장 중요한 요소는 그래프의 정점 및 간선의 개수임. 대표적으로 자율주행 응용의 경우, 입력 그래프의 정점의 개수는 측정 센서 (e.g., LIDAR)의 초당 측정 횟수와 측정 빈도, 센서의 개수가 결정되는 순간 같이 결정됨.}
%     \item \khlc{이때 그래프의 간선은 각 정점마다 가장 가까운 k개의 정점을 연결하는 등의 방법을 통해 생성됨으로, 그래프의 간선의 개수 또한 그래프의 구축 알고리즘과 함께 대략적으로 결정됨.}
%   \end{itemize}
%   \item \khlc{Note: AutoGNN은 UPE와 SCR 모듈 각각이 활용할 수 있는 FPGA 자원의 총량을 고정함으로써 FPGA의 부분적인 재구성이 가능하도록 하였으며, 가능한 모든 하드웨어 구성에 대해 비트스트림을 미리 합성 (synthesis, implementation, export bitstream)하여 FPGA의 메모리에 둠으로써 재구성에 요구되는 시간을 최소화하였음.}
% \end{itemize

\hlA{\noindent\textbf{Overhead of the cost model.}
Evaluating the cost model consists of two steps:
i) evaluating cost-related graph parameters, which are handled by AutoGNN during graph conversion.
ii) computing the costs for all available bitstreams, which is done by the host library.
In our evaluation, the computation of the cost functions took less than 0.1 ms, which is under 0.1\% of the end-to-end latency.}
\markerCommentOnly[-18]{\shortstack{A\#Q1: Overhead \\ of the cost model}}

% \begin{itemize}[leftmargin=*]
%   \item \khlc{소프트웨어의 주요 역할은 입력된 그래프의 크기 (정점, 간선 개수)의 파악 및 최적의 비트스트림 파악임.}
%   \item \khlc{이중 입력된 그래프의 크기를 파악하는 연산은 큰 오버헤드로 작용하지 않음.}
%   \begin{itemize}[leftmargin=*]
%     \item \khlc{첫째, 그래프가 계속 변화하는 경우, 현재까지의 간선 개수와 정점 개수 (최대 VID)를 트래킹함으로써 새로운 간선이 추가될 때마다 이를 업데이트하여 정확한 값을 알 수 있음.}
%     \item \khlc{둘째, 매번 새로운 그래프가 생성되는 응용의 경우, 앞서 설명한 바와 같이 정점/간선의 개수가 센서 시스템과 그래프 구축 알고리즘에 의해 결정되기 때문에, 이를 통해 계산하여 구할 수 있음.}
%     \item \khlc{Note: 해당 연산은 HW 재구성과 관계없이, GPU/FPGA로 그래프 및 그래프 임베딩의 데이터를 전송하는 과정에서, 전송할 데이터의 크기를 알기 위해 반드시 수행되어야 하는 연산임.}
%   \end{itemize}
%   \item \khlc{그래프의 크기를 통해 최적의 비트스트림을 파악하는 연산은 각 비트스트림에 대해 Table 1에 도식된 cost function을 연산하고, 이중 최솟값을 찾으면 됨.}
%   \begin{itemize}[leftmargin=*]
%     \item \khlc{해당 연산은 단순한 곱셈, 나눗셈, 지수-로그 연산으로 이루어져 있기 때문에 CPU에서 매우 빠르게 처리됨을 확인함 (<1ms).}
%     \item \khlc{Note: AutoGNN은 UPE와 SCR이 차지하는 FPGA 자원의 비율을 고정했기 때문에, 두 하드웨어의 비트스트림이 서로 decouple되어 있음. 이에 따라 총 11개 (UPE 5개, SCR 6개)의 비트스트림에 대해 해당 cost function을 연산하면 충분함.}
%   \end{itemize}
% \end{itemize}
